Multidimensional Included and Excluded Sums

This paper presents algorithms for the included-sums and excluded-sums problems used by scientific computing applications such as the fast multipole method. These problems are defined in terms of a $d$-dimensional array of $N$ elements and a binary associative operator~$\oplus$ on the elements. The included-sum problem requires that the elements within overlapping boxes cornered at each element within the array be reduced using $\oplus$. The excluded-sum problem reduces the elements outside each box. The weak versions of these problems assume that the operator $\oplus$ has an inverse $\ominus$, whereas the strong versions do not require this assumption. In addition to studying existing algorithms to solve these problems, we introduce three new algorithms. The bidirectional box-sum (BDBS) algorithm solves the strong included-sums problem in $\Theta(d N)$ time, asymptotically beating the classical summed-area table (SAT) algorithm, which runs in $\Theta(2^d N)$ and which only solves the weak version of the problem. Empirically, the BDBS algorithm outperforms the SAT algorithm in higher dimensions by up to $17.1\times$. The \defn{box-complement} algorithm can solve the strong excluded-sums problem in $\Theta(d N)$ time, asymptotically beating the state-of-the-art corners algorithm by Demaine et al., which runs in $\Omega(2^d N)$ time. In 3 dimensions the box-complement algorithm empirically outperforms the corners algorithm by about $1.4\times$ given similar amounts of space. The weak excluded-sums problem can be solved in $\Theta(d N)$ time by the bidirectional box-sum complement (BDBSC) algorithm, which is a trivial extension of the BDBS algorithm. Given an operator inverse $\ominus$, BDBSC can beat box-complement by up to a factor of $4$.

==> accuracy.tex <==
\section{Accuracy Analysis}\label{app:accuracy}

This section analyzes the \longex and \demalg in terms of the ``sum-depth'', a
measure of numerical accuracy.  Since the excluded-sums problem underlies
scientific computing applications such as the FMM which value numerical
accuracy, lower sum-depth algorithms are preferable because lower sum-depth
corresponds to higher accuracy. Along the way, we will discuss low sum-depth
prefix sums because both the \longex and \demalg depend heavily on prefix sums.

Given a summation algorithm (e.g. reduction, prefix sum), the \defn{sum-depth}
is the longest chain of additions along any path from the inputs to the
output(s).  The worst-case backward error bound of a sum calculation is
proportional to its sum-depth~\cite{Fraser20, higham_paper, BlanHiMa20}.
We generally analyze work, span, and parallelism asymptotically, because
constant factors in these measures are often dominated by machine overheads.  We
express the sum-depth exactly, however, because accuracy is not influenced by
machine performance~\cite{hpec}.

\paragraph{Summation Building Blocks.} The sum-depth of a summation algorithm
may be reduced using tree-like pairwise addition.  For example, the canonical
pairwise reduction that adds all $N$ numbers in a list up in a tree has $\lg N$
sum-depth~\cite{higham_book}. The lowest sum-depth prefix-sum algorithm uses the
Kogge-Stone adder~\cite{KoggeStone73}, which has $\Theta(N \log N)$ work and
$\lg N$ sum-depth on an input of size $N$. In contrast, the canonical
work-efficient upsweep/downsweep prefix sum algorithm has work $\Theta(N)$ but
sum-depth $2\lg N$ on an input of size $N$~\cite{blelloch}.

\paragraph{Prefix Sums.} Since prefix sums are a core subroutine in both
discussed algorithms for excluded sums, we focus our attention on a
work-efficient low sum-depth prefix sum.

\begin{lemma}[Low Sum-depth Prefix Sum]
  Given an input of size $N$, there exists a work-efficient prefix sum
  algorithm, which we will call \accprefix, with $\lg N + 2\lg\lg N$ sum-depth.
\label{lem:prefix-sum-depth}
\end{lemma}

\begin{proof}
  We will describe a low sum-depth prefix sum algorithm called \accprefix
  inspired by the prefix sum implementation from Parlaylib~\cite{BlelAnDh20},
  which divides the input in blocks and proceeds in stages. In the first stage,
  \accprefix divides the input into blocks of size $\lg N$ and performs a
  pairwise reduce on each block in $\Theta(N)$ work and $\lg \lg N$
  sum-depth. In the second stage, \accprefix copies the reduction of each block
  into a temporary array of size $N/\lg N$ and performs the Kogge-Stone prefix
  sum in $\Theta((N/\lg N)\log(N/ \lg N)) = O(N)$ work and
  $\lg (N/\lg N) = \lg N - \lg \lg N$ span. Finally, the third stage propagates
  the result of the prefix sum in the second stage and performs a traditional
  upsweep/downsweep on each block, for $\Theta(N)$ work and $2 \lg \lg n$
  sum-depth.

  Putting it all together, \accprefix has $\Theta(N)$ work and
  $\lg N + 2 \lg \lg N$ sum-depth.
\end{proof}

The corresponding low sum-depth suffix sum \accsuffix is symmetric, so we omit
its discussion.

\paragraph{Excluded-sums Algorithms.} The sum-depths of
the \longex and \demalg follow directly from~\lemref{prefix-sum-depth}.

\begin{theorem}[Box-complement Sum-depth]
  Given a $d$-dimensional tensor of size $N$, the \longex algorithm has
  \boxcompsumdepth sum-depth.
\label{thm:box-comp-sum-depth}
\end{theorem}

\begin{proof}
  The sum-depth over dimension-reduction steps in the \longex is maximized when
  there is a prefix sum along each dimension. Let $s(N)$ be the sum-depth of
  \accprefix on $N$ elements. The prefix along every dimension has sum-depth
  $\sum^d_{i=1} s(n_i)$. From~\lemref{prefix-sum-depth},
$$ \sum^d_{i=1} s(n_i) =  \sum^d_{i=1} \paren{\lg n_i + 2 \lg \lg n_i} = \lg N +
2 \lg lg N. $$

Finally, the box-complement algorithm can add up the $2d$ contributions in a
pairwise reduction, for additional sum-depth $\lg 2d = \lg d + 1$. Therefore,
the total sum-depth of the box-complement algorithm is \boxcompsumdepth.
\end{proof}

Similarly, given a $d$-dimensional tensor of size $N$, the \demalg has
  \cornerssumdepth sum-depth. The analysis is almost exactly the same as the
  box-complement algorithm sum-depth, except that there are $2^d$ contributions
  rather than $2d$.

  \iffalse

\begin{theorem}[Box-complement Sum-depth]
  Given a $d$-dimensional tensor of size $N$, the \longex algorithm has
  \boxcompsumdepth sum-depth.
\label{thm:box-comp-sum-depth}
\end{theorem}

\begin{proof}
There are $d$ dimension reduction steps, and the sum-depth is determined by
maximum sum-depth over all the steps. The maximum sum-depth across steps is
achieved when there is a prefix sum along each dimension. Let $s(N)$ be the
sum-depth of \accprefix on $N$ elements. The prefix along every
dimension has sum-depth $\sum^d_{i=1} s(n_i)$. From~\lemref{prefix-sum-depth},
$$ \sum^d_{i=1} s(n_i) =  \sum^d_{i=1} \paren{\lg n_i + 2 \lg \lg n_i} = \lg N +
2 \lg lg N. $$

Finally, the box-complement algorithm can add up the $2d$ contributions in a
pairwise reduction, for additional sum-depth $\lg 2d = \lg d + 1$. Therefore,
the total sum-depth of the box-complement algorithm is \boxcompsumdepth.
\end{proof}

\fi
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> app-exsum-fig.tex <==
\iffalse
\section{Exsum figures}\label{app:exsum-fig}
\begin{figure*}[htb]
  \begin{center}
    \includegraphics[width=.8\linewidth]{figures/2d-exsum-steps-crop.pdf}
    \end{center}
    \caption{Steps for computing the excluded sum in two dimensions with
      included sums on prefix and suffix sums. The steps are labeled in the
      order they are computed. The prefix \textbf{(a)} and suffix \textbf{(b)}
      steps of computing the $1$-complement perform a prefix and suffix along
      dimension $1$ and an included sum along dimension $2$. The numbers in
      \textbf{(a)},\textbf{(b)} represent the order of subroutines in those
      steps. The prefix \textbf{(c)} and suffix \textbf{(d)} steps of computing
      the $2$-complement perform a prefix and suffix sum on the reduced array,
      denoted by the blue rectangle, from step $\textbf{(a)}$.  The red box
      denotes the excluded region, and solid lines with arrows denote prefix or
      suffix sums along a row or column. The long dashed line represents the
      included sum along each column.}
    \label{fig:2d-exsum-steps}
  \end{figure*}
\fi

==> app-incsum-graveyard.tex <==
\section{Parallel Preliminaries}\label{app:parallel-prelim}

The linguistic model for multithreaded pseudocode from~\cite[Chapter~27]{CLRS}
follows Cilk~\cite{IntelCilkPlus10}. It augments serial code with three
keywords: \defn{spawn}, \defn{sync}, and \defn{parallel}; the last of which
can be implemented with the first two.

The \defn{spawn} keyword before a function call creates nested parallelism. The
\defn{parent} function executes a spawn and can execute in parallel with the
spawned \defn{child} subroutine. Therefore, the code that immediately follows
the spawn may execute in parallel with the child, rather than waiting for it to
complete as in a serial function call. A parent function cannot safely use the
values returned by its children until after a \defn{sync} statement, which
causes the function to wait until all of its spawned children to complete before
proceeding to the code after the sync. Every function also implicitly syncs
before it returns, preventing orphaning.

The spawn and sync keywords denote logical parallelism in a computation, but do
not require parts of a computation to run in parallel. At runtime, a
\defn{scheduler} determines which subroutines run concurrently by assigning them
to different cores in a multicore machine.  Cilk has a runtime system that
implements a provably efficient work-stealing scheduler~\cite{BlumofeJoKu96}.

Parallel loops can be expressed by preceding an ordinary \texttt{for} with the
keyword \defn{parallel}, which indicates that all iterations of the loop may run
in parallel. Parallel loops can be implemented by parallel divide-and-conquer
recursion using spawn and sync. In the work-span model, a parallel loop with $N$
iterations has $\Theta(\log N)$ span.

Given an array $A$ and indices $start \leq end$, let \parprefix$(A, start, end)$
and be the parallel algorithm that computes the prefix sum in the range
$[start, end]$. Similarly, let \parsuffix$(A, start, end)$ be the corresponding
parallel suffix-sums algorithm.


\subsection*{Analysis}

We shall analyze the performance of algorithms for included and excluded sums
using the \defn{work-span model}~\cite[Chapter~27]{CLRS}. The \defn{work} is the
serial running time, or the total time to execute the entire algorithm on a
given input on one processor.  We say that a parallel algorithm is
(asymptotically) \defn{work-efficient} if its work is within a constant factor
of the work of the best serial algorithm for the problem.  The
\defn{parallelism} of an algorithm on a given input is the work divided by the
span.



\clearpage

\section{Included Sums Appendix}\label{app:incsum-par}

\subsection*{1D}



\begin{figure}[t]
\begin{codebox}
  \li \Commnt{\textbf{Input:} List $A$ of size $N$ and}
   \Commnt{ included-sum length $k$.}
  \Commnt{\textbf{Output:} List $A'$ of size $N$ where each }
  \EndCommnt{entry $A'[i] = A[i\rt i+k]$
  for $i = 1, 2, \ldots N$.}
  \Procname{$\onedinc(A, N, k)$}
 \li allocate $\id{A'}$ with $N$ slots
 \li $A_p \gets A; A_s \gets A$
 \li \For $\id{i} \gets 1$ \To $\id{N/k}$ 
 \li \Do \EndCommnt{$k$-wise prefix sum
 along $A_p$} 
 \li \prefix($A_p$, $(i-1)k + 1$, $ik$)
  \li \EndCommnt{$k$-wise suffix sum
along $A_s$ } \label{li:1d-incsum-inner-suf}
 \li \suffix($A_s$,  $(i-1)k + 1$, $ik$)
\End
\li \For $\id{i} \gets 1$ \To $\id{N}$ \label{li:1d-incsum-result} \quad
\EndCommnt{Combine into result }
\li \Do \If $\id{i} \bmod k = 0$
\li \Do $A'[\id{i}] \gets A_s[\id{i}]$
\li \Else
\li $A'[\id{i}] \gets A_s[\id{i}] \oplus A_p[\id{i} + \id{k} - 1]$
\End
\End
\li \Return $A'$
\end{codebox}
\caption{Pseudocode for the 1D included sum.}
\label{fig:incsum-1d-code}
\end{figure}

\begin{lemma}[Correctness in 1D]
    \label{lem:incsum-1d}
    \onedinc solves the included sums problem in 1 dimension.
\end{lemma}

\begin{proof}
  Consider a list $A$ with $N$ elements and box length $k$. We will show that
  for each $x = 1, 2, \ldots, N$, the output $A'[x]$ contains the desired
  sum. For $x \mod k = 1$, this holds by construction. For all other $x$, the
  previously defined prefix and suffix sum give the desired result. Recall that
  $A'\brack{x} = A_p\brack{x + k - 1} + A_s\brack{x}, A_s\brack{x} =
  A\brack{x:\ceil{(x+1)/k} \cdot k}$, and
  $A_p\brack{x + k - 1} = A\brack{\floor{(x + k - 1)/k} \cdot k: x+ k}.$ Also
  note that for all $x \mod k \neq 1$, $\floor{(x + k - 1)/k} = \ceil{(x+1)/k}$.

  Therefore,
  \begin{align*}
    A'[x] & = A_p\brack{x + k - 1} + A_s\brack{x} \\
             & = A \brack{x:\ceil{\frac{x+1}{k}} \cdot k} +
                A \brack{\floor{ \frac{x + k - 1}{k} } \cdot k:x+ k} \\
    & =A \brack{x:x + k}
  \end{align*}
  which is exactly the desired sum.
\end{proof}

\begin{lemma}[Work and Space in 1D]
  \label{lem:incsum-1d-work-space}
  Given an input array $A$ of size $N$ and box length $k$, \onedinc has
  $\Theta(N)$ work and $\Theta(N)$ space.
\end{lemma}

\begin{proof}
  The total work of the prefix and suffix sums is $O(N)$, and the loop that
  aggregates the result into $A'$ has $N$ iterations of $O(1)$ work
  each. Therefore, the total work of \onedinc is $\Theta(N)$. Furthermore,
  \onedinc uses two temporary arrays of size $N$ each for the prefix and suffix,
  for total space $\Theta(N)$.
\end{proof}

\paragraph{In Parallel}
~\appref{parallel-prelim} contains a description of parallel syntax and
constructs.~\figref{incsum-1d-code-par} presents pseudocode for parallelizing
\onedinc.

\begin{figure}[t]
\begin{codebox}
  \li \Commnt{\textbf{Input:} list $A$ of size $N$, box length $k$}
  \Commnt{\textbf{Output:} list $B$ of size $N$ where each entry}
  \EndCommnt{$B[i] = A[i\rt i+k]$ for $i = 1, 2, \ldots N$.}
  \Procname{$\onedinc(A, N, k)$}
 \li \texttt{init} $B[N]$
 \li $A_p \gets A, A_s \gets A$
 \li \Parfor $\id{i} \gets 0$ \To $\id{N/k}-1$ \label{li:1d-incsum-outer}
 \li \Do \EndCommnt{$k$-wise prefix sum
 along $A_p$} 
 \li \parprefix($A_p$, $(i-1)k + 1$, $ik$)
  \li \EndCommnt{$k$-wise suffix sum
along $A_s$ } \label{li:1d-incsum-inner-suf}
 \li \parsuffix($A_s$,  $(i-1)k + 1$, $ik$) \label{li:1d-incsum-inner-suf}
\End
\li \Parfor $\id{i} \gets 1$ \To $\id{N}$ \label{li:1d-incsum-result}
\li \Do \If $\id{i} \mod k \eqeq 1$
\li \Do $B[\id{i}] \gets A_s[\id{i}]$
\li \Else
\li $B[\id{i}] \gets A_s[\id{i}] \oplus A_p[\id{i} + \id{k} - 1]$
\End
\End
\li \Return $B$
\end{codebox}
\caption{Pseudocode for the included sum in 1 dimension in parallel.}
\label{fig:incsum-1d-code-par}
\end{figure}

\begin{lemma}[Span in 1D]
  \label{lem:incsum-1d-span}
  Given an input array $A$ of size $N$ and box length $k$, \onedinc has
  $\Theta(\log N)$ span.
 \end{lemma}

 \begin{proof}
   The loop over the $N/k$ ranged prefix and suffix sums can be run in parallel,
   and the size-$k$ prefix and suffix sums can be replaced with parallel prefix
   and suffix. The resulting span is therefore
   $\Theta(\log (N/k) + \log k) = \Theta(\log N)$. Finally, the loop that adds together
   the relevant prefix and suffix for each coordinate can be parallelized
   parallelized with span $\Theta(\log N)$, for total span $\Theta(\log N)$.
\end{proof}

\subsection*{Higher Dimensions}

Let subroutines \incprerow, \incsufrow, and \incresultrow generalize the ranged
prefix, suffix, and result combination from \onedinc into arbitrary
dimensions. That is, \incprerow, \incsufrow, and \incresultrow take a row as
input and compute the ranged prefix, suffix, or included sum (respectively)
along the specified row.

The subroutines \incprerow, \incsufrow, and  \incresultrow take as input
\begin{itemize}[noitemsep,topsep=2pt]
\item a tensor \tA,
\item a number $i$ of initial dimensions that have been fully reduced so far
  (with default value $i=1$), which will be used in the dimension reduction of
  the box-complement algorithm later,
\item the number of initial dimensions to range over $j$ (the routines perform
  their computation along dimension $j+1$),
\item a row $\vx = (x_1, \ldots, x_j, \rt, x_{j+2}, \ldots, x_\dimension)$,
  and
  \item a box size $\vk = (k_1, \ldots, k_\dimension)$,
\end{itemize}

and compute the ranged prefix, suffix, or included sum (respectively) along the
specified row.

% prefix
\begin{figure}[h]
\begin{codebox}
  \li  \Commnt{\textbf{Input:} Tensor $\tA_p$ ($\dimension$ dimensions, side
  lengths}
   \Commnt{($n_1,
  \ldots, n_{\dimension}$)), dimensions reduced
   up to $\id{i}$,}
  \Commnt {dimensions to take
  points up to $\id{j}$ ($j \geq i$),}
  \Commnt{row defined by coordinate $\vx$, and box size $\vk$.}
  \Commnt{\textbf{Output:} Modify $\tA_p$ to do a ranged prefix sum}
  \Commnt{along dimension $j$  while fixing dimensions}
  \Commnt{up to $i$.}
   \li \EndCommnt{Divide up row in $n_j/k_j$ pieces of size $k_j$ each}
  \Procname{$\incprerow(\tA_p, \id{i}, \id{j}, \id{\vx} =
    (x_1, \ldots, x_d), \id{\vk} = (k_1, \ldots, k_d))$}
  \li \Parfor $\id{l} \gets 0$ \To $\id{n_j/k_j} - 1$
  \li \Do \EndCommnt{$k$-wise prefix sum}
\li \For $\id{m} \gets 2$ \To $\id{k_j}$
along row
\li \Commnt{The serial k-wise prefix is presented here}
\quad\quad \EndCommnt{for clarity, but it can
be any parallel prefix.}
\li \Do $\tA_p[\underbrace{n_1,\ldots, n_{i}}_{\text{$i$}},
\underbrace{x_{i+1},\ldots, x_{j}}_{\text{$j-i$}},$ \\
\li \quad \quad  $lk_{j+1} + m, \underbrace{x_{j+2}, \ldots, x_{\dimension}}_{\text{$d - j-1$}}] \pluseq$ \\
\li $\tA_p[\underbrace{n_1,\ldots, n_i}_{\text{$i$}},
\underbrace{x_{i+1},\ldots, x_{j}}_{\text{$j-i$}},$ \\
\li \quad\quad $lk_{j+1} + m - 1,
\underbrace{x_{j+2}, \ldots, x_{\dimension}}_{\text{$d - j-1$}}]$
\End
\End
\end{codebox}
\caption{Ranged prefix along row (in parallel).}
\label{fig:incsum-presum}
\end{figure}

The ranged suffix along a row is almost exactly the same as the ranged prefix,
so we omit it.

% add into result
\begin{figure}[h]
  \begin{codebox}
      \li \Commnt{\textbf{Input:} Tensor $\tA$ ($\dimension$ dimensions, side
      lengths}
      \Commnt{($n_1,
      \ldots, n_{\dimension}$)) to write the output,
      dimensions reduced}
        \Commnt{up to $\id{i}$, dimensions to take
      points up to $\id{j}$ ($j \geq i$),}
       \Commnt{row defined by coordinate $\vx$, box size
      $\vk$,  ranged prefix}
      \Commnt{and suffix tensors $\tA_p, \tA_s$.}
       \Commnt{\textbf{Output:} Modify $\tA$ with the included sum along}
      \Commnt{the specified row in dimension $j$.}
  \Procname{$\incresultrow(\id{\tA}, \id{i}, \id{j}, \id{\vx} =
    (x_1, \ldots, x_d), \id{\vk} = (k_1, \ldots, k_d), \tA_p, \tA_s)$}
  \li \Commnt{If on a boundary, just assign to the beginning of}
  \Commnt{the k-wise suffix (equal to the sum of k elements}
  \EndCommnt{in this window)}
\li \Parfor $\id{\ell} \gets 1$ \To $\id{n_j}$
\li \Do \If $\ell \mod k_j == 1$
\li \Do $\tA[\underbrace{n_1,\ldots, n_{i}}_{\text{$i$}},
\underbrace{x_{i+1},\ldots, x_{j}}_{\text{$j-i$}}, \ell,
\underbrace{x_{j+2}, \ldots, x_{\dimension}}_{\text{$d - j-1$}}] = $
\li $\tA_s[\underbrace{n_1,\ldots, n_{i}}_{\text{$i$}},
\underbrace{x_{i+1},\ldots, x_{j}}_{\text{$j-i$}}, \ell,
\underbrace{x_{j+2}, \ldots, x_{\dimension}}_{\text{$d - j-1$}}]$
\li \Else \quad \Comment Otherwise, add in relevant prefix and suffix
\li $\tA[\underbrace{n_1,\ldots, n_{i}}_{\text{$i$}},
\underbrace{x_{i+1},\ldots, x_{j}}_{\text{$j-i$}}, \ell,
\underbrace{x_{j+2}, \ldots, x_{\dimension}}_{\text{$d - j - 1$}}] =$
\li \quad $\tA_s[\underbrace{n_1,\ldots, n_{i}}_{\text{$i$}},
\underbrace{x_{i+1},\ldots, x_{j}}_{\text{$j-i$}}, \ell,
\underbrace{x_{j+2}, \ldots, x_{\dimension}}_{\text{$d - j - 1$}}] \oplus$
\li \quad $\tA_p[\underbrace{n_1,\ldots, n_{i}}_{\text{$i$}},
\underbrace{x_{i+1},\ldots, x_{j}}_{\text{$j-i$}}, \ell + k_{j+1} - 1,$
\li \quad \quad $\underbrace{x_{j+2}, \ldots, x_{\dimension}}_{\text{$d - j - 1$}}]$
\End
\End
\End
\End
\end{codebox}
\caption{Computes the included sum along a given row.}
\label{fig:incsum-result}
\end{figure}


\begin{figure}[h]
\begin{codebox}
     \li \Commnt{\textbf{Input:} Tensor $\tA$ ($\dimension$ dimensions, side
     lengths}
     \Commnt{($n_1,
     \ldots, n_{\dimension}$)), dimensions reduced up to $\id{i}$,}
     \Commnt{dimensions to take points up to $\id{j}$ ($j \geq i$),}
     \Commnt{row
     defined by coordinate $\vx$, box size $\vk$.}
     \Commnt{\textbf{Output:} Compute the included sum along}
     \Commnt{dimension $j+1$ in place.}
  % \li Runtime is $O(n^{d-i})$ because the outer for loop has $n^{d-i-1}$ rows
  % that it iterates over and each row takes $O(n)$ to do the presum.
     \Procname{$\incdim(\id{\tA}, \id{i}, \id{j}, \id{\vk} = (k_1, \ldots, k_d))$}
    \li \EndCommnt{Save into temporaries to not overwrite input}
\li Set $\tA_p \gets \tA$ and $\tA_s \gets \tA$
\li \Commnt{Iterate through coordinates by varying}
\Commnt{coordinates in dimensions
$i+1, \ldots, d$}
\EndCommnt{while fixing the first $i-1$ dimensions.}
\li \Parfor \li
$\{\vx = (x_1, \ldots, x_\dimension) \in ( \underbrace{n_1 ,\ldots, n_{i}}_{\text{$i$ }},
\underbrace{:,\ldots, :}_{\text{$j - i$}}, \_,
\underbrace{:, \ldots, :}_{\text{$d - j - 1$}})\}$
\li \Do \Spawn $\incprerow(\tA_p, \id{i}, \id{j}, \id{\vx}, \id{\vk})$
\li $\incsufrow(\tA_s, \id{i}, \id{j}, \id{\vx}, \id{\vk})$
\li \Sync
\li \EndCommnt{Calculate incsum into output}
\li $\incresultrow(\id{\tA}, \id{i}, \id{j}, \id{\vx}, \id{\vk}, \tA_p, \tA_s)$
\End
\end{codebox}
\caption{Computes the included sum along a given dimension in parallel.}
\label{fig:incsum-along-dim-par}
\end{figure}

\begin{figure}[h]
  \begin{codebox}
     \li \Commnt{\textbf{Input:} Tensor $\tA$ ($\dimension$ dimensions), box-lengths $\vk$.}
      \Commnt{\textbf{Output:} Compute the included sum}
     \EndCommnt{in all dimensions in place.}
  \Procname{$\shortinc(\id{\tA}, \id{\vk} = (k_1, \ldots, k_d))$}
 \li $\tB \gets \tA$
\li \For $j \gets 0$ \To $\dimension - 1$
\li \Do $\incdim(\id{\tB}, 0, \id{j}, \vk)$
\End
\li \Return $\tB$
%\li \Comment Included sums in all dimensions is in $A$.
\End
\end{codebox}
\caption{Computes the included sum for the entire tensor.}
\label{fig:incsum-full}
\end{figure}

% \clearpage


\begin{lemma}[Included Sum Computation]
  Let \tA be a tensor and $\tA'$ be the output after
  \incdimfull. For all $x_{j+1} \in [1, n_{j+1}]$,
   \begin{eqnarray*}
 \lefteqn{    \tA'[\, \underbrace{n_1,\ldots, n_{i}}_{\text{$i$}},
    \underbrace{x_{i+1},\ldots, x_{\dimension}}_{\text{$d - i$}}] = } \\
 & &   \tA[\underbrace{n_1,\ldots, n_{i}}_{\text{$i$}},
    \underbrace{x_{i+1},\ldots, x_{j}}_{\text{$j-i$}},
     x_{j+1}:x_{j+1} + k_{j+1}, \\
   & & \quad \quad \underbrace{x_{j+2}, \ldots,
     x_\dimension}_{\text{$d - j-1$}}\,].
     \end{eqnarray*}
\end{lemma}


% \begin{lemma}
  \begin{restatable}[Correctness in Higher Dimensions]{lemma}{incsumcorrectness}
  \label{lem:incsum-correctness}
  Applying \incdim along $i$ dimensions of a $d$-dimensional tensor solves the
  included-sums problem up to $i$ dimensions.
\end{restatable}
  % \end{lemma}

\begin{proof}
  By induction.

  \textbf{Base case: } The one-dimensional case was proven in~\lemref{incsum-1d}.

  \textbf{Inductive Hypothesis:} Let $\tB_i$ be the result of $i$ iterations of the
  above \shortinc algorithm. That is, we do \shortinc along dimensions $1,
  \ldots, i$. Suppose that $\tB_i$ is the included sum in $i$ dimensions.

  \textbf{Inductive Step:} We will show that $\tB_{i+1} = \incdim(\tB_i, 0,
  i+1, \vk)$ % \helen{the $=$ here is too close}
  is the included sum of $i+1$ dimensions. By the induction hypothesis,
  each element of $\tB_i$ is the included sum in $i$ dimensions. Consider any
  valid coordinate $\vx = (x_1, \ldots, x_d)$. The value in $\tB_{i+1}$ at
   \vx is
  \begin{align*}
    \tB_i[\vx] & = \tA[\underbrace{x_1:x_1+k_1, \ldots, x_i:x_i+k_i}_{i
                 },
               \underbrace{x_{i+1}, \ldots, x_d}_{d-i}]
\end{align*}
\begin{align*}
    \tB_{i+1}[\vx] & =   \tA[\underbrace{x_1:x_1+k_1, \ldots,
                     x_i:x_i+k_i}_{i}, \\
    & \quad \quad  x_{i+1}:\ceil{ (x_{i+1}+1)/k_{i+1} } \cdot k_{i+1},
                   \underbrace{x_{i+2}, \ldots, x_d}_{d-i-1}] \\
             & \oplus \tA[\underbrace{x_1:x_1+k_1, \ldots,
               x_i:x_i+k_i}_{i}, \\
& \quad \quad  \floor{ (x_{i+1} + k_{i+1}-1)/k_{i+1} } \cdot k_{i+1}:
               x_{i+1}+ k_{i+1}, \\
             &  \quad  \quad \underbrace{x_{i+2}, \ldots, x_d}_{d-i-1}] \\
                & = \tA[\underbrace{x_1:x_1+k_1, \ldots,
               x_{i+1}:x_{i+1}+k_{i+1}}_{i+1}, \\
           &   \quad  \quad  \underbrace{x_{i+2}, \ldots, x_d}_{d-i-1}]
  \end{align*}
\end{proof}

  \begin{restatable}[Work and Space of Included Sum]{lemma}{incsumwork}
% \begin{lemma}[Work of Included Sum]
  \label{lem:incsum-dim-work}
  \incdimfull has \\ \incdimwork work and takes $\Theta(N)$ space.
\end{restatable}
% \end{lemma}


\begin{proof}
  The loop over points in $\incdim$ has
  $\paren{\prod_{\ell={i+1}}^{\dimension} n_\ell}/n_{j+1}$ iterations over
  dimensions $i+1, \ldots, j-1, j, j+2, \ldots, \dimension$. Each subroutine
  call has work $O(n_{j+1})$, for total work
  $O\paren{\prod_{\ell=i+1}^{d} n_\ell}$. Just as in the one-dimensional case,
  \incdim takes $\Theta(N)$ space because it uses two temporaries of size $N$
  for the prefix and suffix.
\end{proof}


\begin{lemma}[Span of Included Sum]
    \label{lem:incsum-dim-span}
   \incdimfull has \incdimspan span.
\end{lemma}

\begin{proof}
  The loop over coordinates in \incdim has
  $\prod_{\ell={i+1}, \ell\neq {j+1}}^{\dimension} n_\ell$ iterations
  which can be done in parallel, for span
  $$\Theta\paren{\log\paren{\prod\limits_{\ell={i+1}, \ell\neq {j+1}}^{d} n_\ell}} =
  \Theta\paren{\sum\limits_{\ell={i+1}, \ell\neq {j+1}}^{d}\log n_\ell}\ .$$

  The subroutines \incprerow and \incsufrow are logically parallel and have
  equal span, so we will just analyze the ranged prefix. The outer loop of \\
  \incprerow can be parallelized, and the inner loop can be replaced with a
  parallel prefix. Therefore, the span of the ranged prefix for each row along
  dimension $j+1$ is
  $$\Theta(\log(n_{j+1}/k_{j+1}) + \log k_{j+1}) = \Theta(\log n_{j+1})\ .$$

  Finally, calculating the contribution to the output for each of the outer loop
  iterations in \incresultrow can be parallelized, for span $O(\log n_{j+1})$.
  Therefore, the total span is

  \begin{align*}
     \Theta\paren{ \paren{ \sum_{\ell={i+1}, \ell\neq {j+1}}^{d}\log n_\ell } + \log  n_{j+1} + \log n_{j+1}} =  \\
    \quad \Theta\paren{\log \paren{\prod_{\ell = i+1}^{d}
        n_\ell}}.
    \end{align*}
\end{proof}

\begin{corollary}
    \label{cor:incsum-full-span}
    \shortinc has \shortincspan span.
  \end{corollary}



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> exsum-figs.tex <==
\begin{figure*}[t]
  \begin{center}
    \includegraphics[width=.7\textwidth]{figures/3d-exsum-regions-crop.pdf}
    \end{center}
    \caption{An example of the recursive box-complement in three dimensions with
       dimensions labeled $1, 2, 3$. The figures \textbf{(a)}, \textbf{(b)}, and
      \textbf{(c)} illustrate the $1$-, $2$-, and $3$-complement,
      respectively. The blue region represents the coordinates inside the box,
      and the regions outlined by dotted lines represent the partitions defined
      by~\corref{excl-components}. For each partition, the face against the edge
      of the tensor is highlighted in green.}
  \label{fig:3d-exsum-regions}
\end{figure*}


==> incsum-code.tex <==
\helen{The main focus of this work is multidimensional included and excluded
  sums.} Computing the included sum along an arbitrary dimension is almost
exactly the same as computing it along 1 dimension in terms of the underlying
ranged prefix and suffix sums.  We sketch a function \shortinc % (full details
% in~\figref{incsum-full} in~\appref{incsum-par})
that generalizes \onedinc to
arbitrary dimensions.

\iffalse
% \paragraph{Correctness and Performance.}
Since the box-complement algorithm for strong excluded sums in~\secref{exsum}
requires \shortinc as a subroutine along arbitrary dimensions after dimension
reduction, we first define a function called \incdim
% (\figref{incsum-along-dim-par} in~\appref{incsum-par}).
\incdim computes the included sum for each row along a specified dimension after
dimension reduction. Let \tA be a $d$-dimensional tensor, $\vk$ be a box size,
$i$ be the number of reduced dimensions so far, and $j$ be the dimension to
compute the included sum along such that $j > i$. \incdimfull computes the
included sum along the $j$th dimension for all rows
$\paren{\, n_1,\ldots, n_{i}, \rt,\ldots,\rt \,}$.  That
% $\smallparen{\, n_1,\ldots, n_{i}, \rt,\ldots,\rt\,}$.  That
is, for each coordinate
$\vx = \smallparen{\, n_1,\ldots, n_{i}, x_{i+1},\ldots, x_{\dimension}\,}$, the
output tensor $\tA'$ contains the included sum along dimension~$j$:
% \squeezeup
\begin{multline*}
  \tA'\smallbrack{\vx} =
  \bigoplus \tA[\underbrace{n_1,\ldots, n_{i}}_{\text{$i$}},  \underbrace{x_{i+1},\ldots, x_{j}}_{\text{$j-i$}}, \\
  x_{j+1}\rt x_{j+1} + k_{j+1}, \underbrace{x_{j+2}, \ldots,
    x_\dimension}_{\text{$d - j-1$}}].
\end{multline*}

\incdimfull takes \incdimwork time because it iterates over
$\paren{\prod_{\ell={i+1}}^{\dimension} n_\ell}/n_{j+1}$ rows and runs in
$\Theta(n_{j+1})$ time per row. It takes $\Theta(N)$ space using the same
technique as \onedinc.
\fi


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> incsum-proofs.tex <==
% \paragraph{Solving the Included-sums Problem.}
Overall, \shortinc computes the
full included sum of a tensor with $N$ elements in $\Theta(dN)$ time and
$\Theta(N)$ space by performing \incdim along each dimension in turn. That is,
calling \incdimfull $d$ times with $i = 0$ and $j = 1, \ldots, \dimension$ solves the
included-sums problem.
% ~\figref{2d-incsum} shows an example of using \shortinc
% to solve the included-sums problem in 2 dimensions.

Although we cannot directly use \shortinc to solve the strong excluded-sums
problem, the next sections demonstrate
% we will demonstrate in~\secref{boxcomp}
how to use \incdim as a key
subroutine in the box-complement algorithm for strong excluded sums.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> parallel.tex <==
\section{Parallelizing the Box-complement Algorithm}\label{app:parallel}

This section shows that, given a $d$-dimensional tensor $\tA$ with size
$N = n_1\cdots \ldots \cdot n_d$, the box-complement algorithm
solves the excluded-sums problem in \boxcompspan span.~\appref{parallel-prelim}
formalizes the parallel constructs used in the pseudocode and proofs in
~\appreftwo{incsum-par}{exsum-par}.


Since the analysis of the span of the main subroutines in the \longex algorithm
is very similar to the analysis of their work, we will omit it and summarize the results
in~\tabref{work-span}.~\appref{incsum-par} contains the formal statements and
proofs.

\begin{table*}[b]
\centering
\begin{tabular}{ lll }
 Subroutine & Work & Span \\ \hline
 \predimfull & \predimwork & \predimspan \\
  \incdimfull & \incdimwork & \incdimspan \\
  \addcontrib & \addcontribwork & \addcontribspan \\
  \hline
\end{tabular}
\caption{Work and span of the main subroutines in the box-complement algorithm.
  The parameter $i$ in \predimfull and \incdimfull represents the number of
  dimensions reduced so far.  The parameter $i$ in \predimfull and $j$ in
  \incdimfull represent the dimension to perform the function along.  }
\label{tab:work-span}
\end{table*}

% \paragraph{Parallelizing the Box-complement Algorithm.}

Parallelizing the \longex algorithm is a matter of replacing its main
subroutines with their parallel versions. The analysis is similar to the proof
of the work of \boxcomp in~\thmref{box-comp-work}.

\begin{theorem}[Box-complement Span]
  \label{thm:exsum-span}
  Given a $d$-dimensional tensor $\tA$ of size $N = n_1 \cdots n_d$,
  \boxcomp has \boxcompspan span.
\end{theorem}

\begin{proof}
  The span of each dimension-reduction step $i \in \{1, \ldots, d\}$ is the sum
  of the spans of the prefix sum along dimension $i$, $d-i$ included sum steps
  with dimensions up to $i-1$ fixed, and adding into the contribution.
  That is, the span is
 $$\Theta\paren{\sum\limits_{i=1}^{d} \brack{
     \underbrace{\paren{\sum\limits^{d}_{j=i}\paren{\sum\limits^{d}_{\ell =
             j}\log n_\ell}}}_{\text{prefix and included sum}} + \underbrace{
       \log N }_{\text{add contrib}}}} = \Theta\paren{d^2\log N}.$$
\end{proof}

Therefore, the parallelism of $\boxcomp$ on a tensor of size $N$ is $\Theta(dN /
d^2 \log N) = \boxcomppar$.
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

